S4G: Amodal Single-view Single-Shot SE(3) Grasp Detection in Cluttered Scenes

Grasping is among the most fundamental and long-lasting problems in robotics study. This paper studies the problem of 6-DoF(degree of freedom) grasping by a parallel gripper in a cluttered scene captured using a commodity depth sensor from a single viewpoint. We address the problem in a learning-based framework. At the high level, we rely on a single-shot grasp proposal network, trained with synthetic data and tested in real-world scenarios. Our single-shot neural network architecture can predict amodal grasp proposal efficiently and effectively. Our training data synthesis pipeline can generate scenes of complex object configuration and leverage an innovative gripper contact model to create dense and high-quality grasp annotations. Experiments in synthetic and real environments have demonstrated that the proposed approach can outperform state-of-the-arts by a large margin.

==> [Arxiv]Grasp Proposal/approach.tex <==
\section{Problem Setting}
We denote the single-view point cloud by $\mathbf{P}$ and the gripper description by $\mathbf{G}$. A parallel gripper can be parameterized by the frame whose origin lies at the middle of the line segment connecting two figure tips and orientation aligns with the gripper axes. We therefore denote a grasp configuration as $c=(\mathbf{h}, s_{\mathbf{h}})$, where $\mathbf{h} \in \mathbb{SE}(3)$ and $s_{\mathbf{h}} \in \mathbb{R}$ is a score measuring the quality of $\mathbf{h}$.

% Sec.~\ref{sec:network} describes our single-shot learning network. Note that our usage of network is different from existing 6-DoF grasping methods. For example, \cite{ten2017grasp} uses networks to assess grasp proposals, which are sampled from $\mathbb{SE}(3)$ by some heuristically designed sampler. We call the traditional pipeline as two-stage. However, designing grasp proposal is not easy,  especially the space of $\mathbb{SE}(3)$ is indeed quite large ($6$-dimensional). We, therefore, introduce a single-shot pipeline that learns to generate grasp proposals. Like single-shot object detectors (e.g., YOLO \cite{redmon2016you} and SSD\cite{liu2016ssd}), our pipeline takes the single-view point cloud as input, and assigns at each point two attributes. The first attribute is a good grasp (if exists) associated by inverse indexing, and the second attribute is the predicted grasp quality score of the grasp. 

% To generate the densely labeled training data for amodal grasp proposal, we seek to train the network using synthetic data that are physically plausible (Sec.~\ref{sec:data_generation}). We use MuJoCo to create synthetic scenes by randomly throwing in CAD models of objects. This scene is captured by a virtual depth sensor as a point cloud. The key of training data synthesis is to generate per-point labels. We propose a simple yet effective gripper contact model to generate good grasps and associate these grasps to the point cloud, and we assess their qualities based on force closure, object/scene collision avoidance, and perception/actuation noises. 

% At inference time, we sample high quality grasps based on the proposals of the network (Sec.~\ref{sec:grasp_generation}). 


\begin{figure}[t!]
\centering
\setlength{\belowcaptionskip}{-0.6cm}
\vspace{-0.4cm}
\includegraphics[width=0.6\textwidth]{imgs/data_generation.pdf}
\caption{Flowchart of scene grasp dataset generation.}
\label{fig:data_generation}
\end{figure}

\section{Training Data Generation}
\label{sec:data_generation}
% \hao{roughly introduce that (1) we need to generate a scene of objects; (2) we need to assign what labels at each point in the scene. then, introduce (1) what scores can be obtained by just analyzing an object, and (2) what scores have to be obtained from the scene. finally, introduce the robustness score.}

To train our \net, a large scale dataset capturing cluttered scenes, with viable grasps and quality scores as groundtruth, is indispensable. Fig.~\ref{fig:data_generation} illustrates the training data generation pipeline. We use the YCB object dataset~\citep{calli2015ycb} for our data generation. Since \net~directly takes a single-view point cloud from the depth sensor as input and outputs collision-free grasps in a densely-cluttered environment, we need to generate such scenario with complete scene point cloud and corresponding partially observed point cloud. Each point in the point cloud is assigned with serval grasps which will be introduced in Sec~\ref{sec:scene_analysis} and each ground truth grasp has a $\mathbb{SE}(3)$ pose, an antipodal score, a collision score, an occupancy score, and a robustness score, which we will introduce later. On the other hand, the scene point cloud does not interact with the network explicitly, but it serves as a reference to evaluate grasps in the point cloud.

% Since the $\mathbb{SE}(3)$ grasp pose, antipodal score, and occupancy score solely depend on individual objects and are constant during the scene generation, they can be first computed from single object, cached into viable grasp set and will be integrated into the scene later. In contrast, the collision score can be only obtained from the scene. Finally, a robustness score will be calculated based on all the other scores, which represents the expected quality of a grasp under execution and sensing errors. 


\subsection{Gripper Contact Model}
% \hao{figure is needed}

% \hao{need formula and algorithm}

% \hao{need to argue why this is a good model}

% \hao{need to give a computational complexity analysis}
\begin{wrapfigure}{r}{0.35\textwidth}
\includegraphics[width=0.35\textwidth]{imgs/contact_model.pdf}
\caption{Illustration of Gripper Contact Model}
\label{fig:contact_model}
\end{wrapfigure}

Vast literature exists to find regions suitable to grasp by analyzing the 3D geometry~\cite{sahbani2012overview}. Among these methods, force closure has been widely used to synthesize grasps and can be reduced into calculating angles between face normals, known as antipodal grasp \cite{nguyen1988constructing, chen1993finding}. Here we introduce our gripper contact model based on force closure analysis to find feasible grasps. 


% Modeling the gripper is of vital importance to generate accurate and successful grasp poses. In our pipeline, we build the Gripper Contact Model to address the interactive problem between gripper and object, which has always been left out of consideration in many other works.

To be more specific, we first detect all possible contact pairs with high antipodal score $s_{\mathbf{h}}^a = \mathbf{cos}(\alpha_1)\mathbf{cos}(\alpha_2)$, where $\alpha_i$ is the angle between the outward normal and the line connecting two contact points. As illustrated in Fig.~\ref{fig:contact_model}, for each contact pair ($p_{i}$, $p_{j}$), the normal $\mathbf{n}_{i}$ at point $p_{i}$ is smoothed with radius $r$mm. Note that this step is important to grasp objects of rugged surface with high-frequency normal variation. However, we do not directly use a ball query to query its neighbors, which will lead to undesirable results at corners and edges. Instead, we remove the neighbors which has a distance along the normal direction ( calculated as $r_i^k=|(\mathbf{p}_i^k-\mathbf{p}_i)\cdot \frac{\mathbf{n}_i}{|\mathbf{n}_i|}|$) larger than $3$mm in the query ball of radius $r$ for normal calculation, where $\mathbf{p}_i^k$ is the $k$-th neighbor of point $i$. 

These two hyper-parameters have definite physical meaning, which is distinct from the approach to obtain the gripper contact model hyper-parameters in GPD~\citep{ten2017grasp} through extensive parameter tuning. As shown in Fig.~\ref{fig:contact_model}, our gripper will only interact with the object by its soft rubber pad, which allows deformation within $3$mm. And the normal smoothing radius is set as the gripper width $r=23$mm. 

In fact, our gripper model has clear advantage over Darboux frame based methods, especially at rugged surfaces and flat surfaces. For rugged surfaces, there is no principled way to decide the radius for normal smoothing, since the radius is not only relevant to the gripper, but also to the object to grasp. For flat surfaces, the principal curvature directions are under-determined. In practice, we do observe issues for these cases. For example, for plates and mugs, Darboux frame based method will likely to fail in generating a successful grasp pose for the thin wall. 

Besides the direction of contact force, we also consider the stability of the grasp. The occupancy score $s_{\mathbf{h}}^o$, which represents the volume of object within the gripper closing region $\mathbf{R(c)}$, is calculated by
\begin{equation} \label{anti}
   s^{o}_{\mathbf{h}} = \min \{ ln(| \mathbf{P_{close}}|), 6 \} ,\quad \mathbf{P_{close}} = \mathbf{R(c)} \cap \mathbf{P},
\end{equation}
where $\mathbf{P_{close}}$ is the number of points within closing region. If $s^{o}_{\mathbf{h}}$ is small, the gripper contact analysis will be unreliable. To make sure that the point cloud occupancy can correctly represent the volume, we down-sample the point cloud using voxel grid filter with a leaf size of $5$mm. 

% \subsection{Generating Occupancy Scores by Object Analysis}
% \label{sec:score}
\subsection{Physically-plausible Scene Synthesis from Objects}

Since our network is trained on synthesis data and directly applied to real world scenarios, it is necessary to generate training data closer to reality both physically and visually.

We need physically-plausible layouts of various scenes where each object should be in equilibrium under gravity and contact force. Therefore, we adopt MuJoCo engine~\cite{todorov2012mujoco} and V-HACD\citep{vhacd} to generate scenes where each object is in equilibrium. Objects initialized with random elevation and poses fall onto a table in the simulator and converge to static equilibrium due to friction. We record the poses and positions of objects and reconstruct the 3D scene.(Fig.~\ref{fig:data_generation})

Beside scene point cloud, we also need to generate viewed point clouds that will feed into the neural network. To simulate the noise of depth sensor, we apply a noise model on the distance from camera optical center to each point as $\Tilde{D}_{o,p} = (1+\mathcal{N}(0,\sigma^2))D_{o,p}$,
where $D_{o,p}$ is the noiseless distance captured by a ray tracer and $\Tilde{D}_{o,p}$ is the distance used to generate viewed point clouds. We employ $\sigma=0.003$ in this paper.


\subsection{Robustness Grasp Generation by Scene Analysis}
\label{sec:scene_analysis}

Given the scene point cloud, we can do collision detection for each grasp configurations. Collision score $s_{\mathbf{h}}^c$ is a scene-specific boolean mask indicating the occurrence of collision between the proposed gripper pose and the complete scene. As shown in our experiment, our network can better predict collision with invisible parts.

It is a common case that robot end-effector can not move precisely to a given pose due to sensor noise, hand-eye calibration error and mechanical-transmission noise. To perform a successful grasp under imperfect condition, the proposal grasp should be robust enough against gripper's pose uncertainty. In this paper, we add a small perturbation to the $\mathbb{SE}(3)$ grasp pose and evaluate the antipodal score, occupancy score and collision score for the perturbed pose. The final scalar score of each grasp can be derived as:
\begin{equation}
    s_{\mathbf{h}} = \min_j [s^a_{\mathbf{h}_j} s^o_{\mathbf{h}_j} s^c_{\mathbf{h}_j}], \quad {\mathbf{h}_j}=\mathbf{exp(\hat{\xi})}\textbf{h},
\end{equation}
where $\mathbf{\hat{\xi}} \in \mathfrak{se}(3)$ is the pose perturbation and $ \mathbf{exp}$ is the exponential mapping. The final viewed point cloud with ground truth grasps and scores will serve as training data for our \net.


% \begin{wrapfigure}{r}{0.45\textwidth}
% \begin{subfigure}[b]{0.20\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{imgs/scene.pdf}
%     \caption{Scene Point Cloud (before downsample)}
%     \end{subfigure}
%     \hfill
% \begin{subfigure}[b]{0.20\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{imgs/view.pdf}
%     \caption{Viewed Point Cloud}
% \end{subfigure}
% \caption{}
% \end{wrapfigure}

% REUSABLE TEXT:
% Figure.~\ref{fig:data_generation} illustrates the pipeline of our dataset generation pipeline. For each point in one point cloud, it is associated with three attributes: collision-free viable grasp, grasp quality score, and practicable removal directions.
% We use the YCB object dataset~\citep{calli2015ycb}, which is collected using a 3D scanner, for our data generation. The viable grasp set is generated using gripper contact model and robustness score as describe below. In order to make our network generalize well, the synthetic data we generate for training should resemble the real world. Therefore, we adopt MuJoCo~\cite{todorov2012mujoco}, a physics simulator, to generate physically feasible layouts. Firstly, a few objects are sampled from the object shape database, which are put in the simulator with random elevation and poses; then all the objects begin to fall onto a table in the simulator and converge to static equilibrium due to friction; finally, we record the poses and positions of objects and reconstruct the 3D scene with their 3D shapes(Fig.~\ref{fig:generated_scene}).  We fetch the viable grasps with corresponding score from the closest point of objects in the scene, and filter out grasps colliding with surroundings.
% Another key factor which effects the grasping success rate especially for dense clutters, is whether the object of interest collides with other objects during removal. We use MuJoCo to detect collision for given removal directions and record practicable ones.
% % To address the challenge of 6-DoF grasp prediction given visual input, a large scale dataset with viable grasps and corresponding scores is indispensable. Since our \net directly takes point cloud as input and outputs the best gripper configuration nearby for every single point as well as the quality of this grasp, the dataset should consist of point-wise metrics that can determine the success of grasping.
% 
% % First, we need physically feasible layouts of various scenes where each object should be in equilibrium under gravity and contact force, which can better represent the realistic scenario. Since our network is expected to find collision free grasp in a cluttered scene, using steady-state placement can also be beneficial for learning the implicit physics. Consider a simple table arena where a large box leans against a small ball, as illustrated in Figure \ref{??}. If the camera is not able to see the ball due to occlusion, the generated grasp may collide with it and then make the box move, which can eventually lead to failure. However, if the training data is physics feasible, the network can learn that there must be something behind the box and try to avoid collision with the underlying object. To create such placement, we adopt MuJoCo physics engine \cite{todorov2012mujoco} to generate scenes where each object is in equilibrium. All the objects are initialized with random elevation and pose. Subject to friction loss, the velocity will get to zeros, and we record the pose of these final states.
% 
% \begin{wrapfigure}{r}{0.4\textwidth}
% \missingfigure[width=0.4\textwidth]{}
% % \includegraphics[width=0.4\textwidth]{imgs/data_generation.pdf}
% \caption{Comparison of generated successful grasps of objects with thin structure.}
% \label{fig:generated_grasp}
% \end{wrapfigure}
% 
% \textbf{Robustness Score}
% 
% In real-life applications, the actual executed grasp may deviate from the detected one due to sensor error, calibration error, or motor error, which makes a successful grasp into a failure. We, therefore, use robustness score to  handle this problem: for each viable grasp, its score is computed by smoothing the scores of its neighbor grasps
% \begin{equation}
%     s_{\textbf{h}_i} = \sum_{\textbf{h}_j\in Q(\textbf{h}_i)}w_js'_{\textbf{h}_j},
% \end{equation}
% where $Q(\textbf{h}_i)$ denotes the neighborhood of $\textbf{h}_i$, and $s'_{\textbf{h}_j}$ is the grasp quality score from the gripper contact model.

\section{Single-Shot Grasp Generation}
\label{sec:network}
\subsection{PointNet++ based Grasp Proposal}
% \subsubsection{Architecture}
\begin{figure}[tbp]
\setlength{\belowcaptionskip}{-0.5cm}
\centering
    \includegraphics[width=\linewidth]{imgs/network_architecture.pdf}
    \caption{Architecture of Single-Shot Grasp Proposal Network based on PointNet++~\citep{qi2017pointnet++}. Given the scene point cloud, our network first extracts hierarchical point set features by progressively encoding points in larger local regions; then the network propagates the point set features to all the original points using inverse distance interpolation and skip links; finally it predicts one 6-DoF grasp pose $\textbf{h}_i$, and one grasp quality score $s_{\textbf{h}_i}$ of every point. }
    \label{fig:architecture}
\end{figure}
We design the single-shot grasp proposal network based on the segmentation version of PointNet++, which has demonstrated state-of-the-art accuracy and strong robustness over clutter, corruption, non-uniform point density \cite{qi2017pointnet++}, and adversarial attacks \cite{liu2019extending}. 

Figure.~\ref{fig:architecture} demonstrates the architecture of \net, which takes the single-view point cloud as input, and assigns each point two attributes. The first attribute is a good grasp (if exists) associated to the point by inverse indexing, and the second attribute is the quality score of the stored grasp. The generation of the grasp and quality score can be found in Sec.~\ref{sec:scene_analysis}.
%Like single-shot object detectors (e.g., YOLO \cite{redmon2016you} and SSD\cite{liu2016ssd}), 

The hierarchical architecture not only allows us to extract local features and predict reasonable local frames when the observation is partial and noisy, but also combines local and global features to effectively infer the geometry relationship between objects in the scene.

% \subsubsection{Frame prediction}
Compared with sampling and grasp classification~\cite{ten2017grasp, liang2019pointnetgpd}, the single-shot 6-DoF grasp direct regression task is more challenging for networks to learn, because widely adopted rotation representations such as quaternions and Euler angles are discontinuous. In this paper, we use a 6D representation of the 3D rotation matrix because of its continuity~\citep{zhou2018continuity}: for every $\mathbf{R} \in \mathbb{SO}(3)$, it is represented by $\mathbf{a} = \left[ {\mathbf{a}_1}, {\mathbf{a}_2} \right]$, $\mathbf{a}_1,\mathbf{a}_2 \in \mathbb{R}^3$, such that the mapping $f:\mathbf{a}\rightarrow\mathbf{R}$ is
\begin{equation}
\begin{array}{l}
\mathbf{R}=\left[\mathbf{b}_1, \mathbf{b}_2, \mathbf{b}_3\right]\\
\mathbf{b}_1=N\left(\mathbf{a}_1\right)\\
\mathbf{b}_2=N\left(\mathbf{a}-\left\langle \mathbf{a}_2,\mathbf{b}_1\right\rangle \mathbf{b}_1\right)\\
\mathbf{b}_3=\mathbf{b}_1 \times \mathbf{b}_2,
\end{array}
\end{equation}
where $N()$ denotes the normalization function. Because the gripper is symmetric with respect to rotation around the $x$ axis, we use a loss function which handles the ambiguity by considering both correct rotation matrices as ground truth options. Given the groundtruth rotation matrix $\mathbf{R}_{GT}$, we define the rotation loss function $L_{rot}$ as
\begin{equation}
\begin{array}{l}
L_{rot} = \underset{i \in \left\{0, 1\right\}}{\textrm{min}}\|f(\mathbf{a}_{pred}) - \mathbf{R}^{(i)}_{GT}\|^2  \\
\mathbf{R}^{(i)}_{GT} = \mathbf{R}_{GT} \begin{bmatrix}1&0&0\\0&\textrm{cos}(\pi i)&0\\0&0&\textrm{cos}(\pi i)\end{bmatrix}
\end{array}
\end{equation}

The prediction of translation vectors is treated as a regression task and the $L_2$ loss is applied. By dividing the groundtruth score into multiple levels, the grasp quality score prediction is treated as a multi-class classification task, and a weighted cross-entropy loss is applied to handle the unbalance between positive and negative data. 
We only supervise the pose prediction for those points assigned with viable grasps and the total loss is defined as:
\begin{equation}
L = \sum_{\mathbf{P}_v}{\left(\lambda_{rot} \cdot L_{rot}  + \lambda_{t} \cdot L_{t} \right)} + \sum_{\mathbf{P}_{s}}{\left(\lambda_{s} \cdot L_{s}\right)},
\label{eq:loss}    
\end{equation}
where $\mathbf{P}_v, \mathbf{P}_s$ represent the point set with viable grasps and the whole scene point cloud, respectively. $\lambda_{rot}, \lambda_{t}, \lambda_{s}$ are set to 5.0, 20.0, 1.0 in experiments.

\subsection{Non-maximum Suppression and Grasp Sampling}
\label{sec:grasp_generation}

% Our network are able to generate diverse grasps in one forward pass, from which a subset are chosen to execute(Algorithm.~\ref{alg:grasp_selection}). 
Algorithm.~\ref{alg:grasp_selection} describes the strategy to choose one grasp execution $\textbf{h}$ from the network prediction $\mathcal C$.
\begin{wrapfigure}[20]{R}{0.5\textwidth} %<-- Wrapfigure covers 6 lines
\begin{footnotesize}
  \begin{algorithm}[H]                %<-- Remove float environment
    \SetCustomAlgoRuledWidth{0.45\textwidth}  %<-- For aesthetics  
    \caption{NMS and Grasp sampling}
    \textbf{Input: } Prediction $\mathcal C$: $\left\{ (\textbf{h}_i, s_{\textbf{h}_i})\right\}$ \\
    \textbf{Export: } Grasp Execution: $\textit{h}$ \\
  \begin{algorithmic}
  \STATE Executable Grasps $\mathcal H = \{\}$
  \STATE {$Sort$ $\left\{ (\textbf{h}_i, s_{\textbf{h}_i}\right\}$ $by$ $s_{\textbf{h}_i}$}
  \STATE {$i = 0$}
  \WHILE{$\mathcal Length(\mathcal H) < N$}
  \IF {$(Collision == False)$ and $\underset{min}{\textbf{h}_k \in \mathcal H}dist(\textbf{h}_i, \textbf{h}_k) > \epsilon$}
  \STATE {$Add$ ${ (\textbf{h}_i, s_{\textbf{h}_i})}$ to ${\mathcal H}$}
  \ENDIF
  \STATE {$i = i+1$}
  \ENDWHILE
  \STATE $p_k = \dfrac{g(s_{\textbf{h}_k})}{\displaystyle\sum_l{g(s_{\textbf{h}_l})}}$ for ${\textbf{h}_k} \in \mathcal{H}$
  \WHILE{Motion planning fails}
  \STATE {Sample $\textit{h}$ according to \{$p_k$\}}
  \ENDWHILE
  
  \end{algorithmic}
  \label{alg:grasp_selection}
  \end{algorithm}
\end{footnotesize}
\end{wrapfigure}

Because the network generates one grasp for each point, there are numerous similar grasps in each grasp's neighborhood and we use non-maximum suppression (NMS) to select grasps $\textbf{h}$ with local maximum $s_{\textbf{h}_i}$ to generate executable grasp set $\mathcal H$. Then weighted random sampling is applied to sample one grasp to execute according to its grasp quality score.

% \begin{table}[tb]
% \begin{footnotesize}
% \setlength{\belowcaptionskip}{-0.5cm}
% \vspace{-0.4cm}
% \renewcommand\arraystretch{1.2}
%     \centering
%     \begin{tabular}{r|cc|cc}
%         \toprule
%         &\multicolumn{2}{c|}{\textbf{w/o Noise}} &\multicolumn{2}{c}{\textbf{ w/ Noise}} \\
%         \hline
%         & Ant. Score    & Collision-free &   Ant. Score    & Collision-free \\
%         \hline
%         GPD (3 channels)   &  0.5947 &  \textbf{47.07\%} &  0.5802  & 40.00\%    \\
%         GPD (12 channels)   &  0.5883  &  45.27\%  &  0.5946  & 40.44\%    \\
%         PointNetGPD    &  0.5718   &  42.41\%  & 0.6376   &  41.17\%   \\
%         \hline
%         Ours & \textbf{0.7364}    & 47.02\%  &\textbf{0.7354}  & \textbf{53.32\%} \\
%         \bottomrule   
%     \end{tabular}
%     \caption{Comparison of grasp quality on simulation data.}
%     \label{tab:simul}
% \end{footnotesize}
% \end{table}



==> [Arxiv]Grasp Proposal/experiments.tex <==


\section{Experiments}
\subsection{Implementation Details}
 The input point cloud is first preprocessed, including workspace filtering, outliers removal, and voxel grid down-sampling. For training and validation, we sample $\frac18N$ points from the point set with viable grasps, $\frac78N$ from the remaining point set, and integrate them as the input of the network. For evaluation, we sample $N$ points at random from the preprocessed point cloud. $N$ is set to 25600 in our experiments. We implement our network in PyTorch, and train it using Adam~\citep{kingma2014adam} as the optimizer for 100 epochs with the initial learning rate $0.001$, which is decreased by $2$ every $20$ epochs. 


\subsection{Superiority of $\mathbb{SE}(3)$ grasp}
We first evaluated the grasp quality performance of our proposed network on simulated data.
To demonstrate the superiority of $\mathbb{SE}(3)$ grasp over 3/4 DoF grasp, here we give a quantitative analysis over 6k scene with around 2.6M generated grasps (Fig. \ref{fig:6dadvantage}). In our experiments, grasps are uniformly divided into 6 groups according to the angle between the approach vector and vertical direction in the range of ($0^{\circ}, 90^{\circ}$). We use the recall rate as metric which are defined as the percentage of objects that can be grasped using grasps between vertical and certain angle. We evaluate the recall rate at scenes of three different densities: simple (1-5 objects presented in the scene), semi-dense (6-10 objects) and dense (11-15) objects. The overall recall rate is the weighted average of the three scenes. We find that only $63.38\%$ objects can be grasped by nearly vertical grasps ($0^{\circ}, 15^{\circ}$). With the increase of scene complexity, the advantage of $\mathbb{SE}(3)$ grasp becomes more remarkable.

\begin{wrapfigure}{R}{0.40\textwidth}
    \centering
    \setlength{\belowcaptionskip}{-0.5cm}
    \includegraphics[width=1\linewidth]{imgs/6dadvantage.pdf}
    \caption{Results of simulated experiment on the recall rate of different grasp. The X-axis is the angle between the approach vector and vertical direction. The angle of absolute 3/4 DoF grasp is $0^{\circ}$}
    \label{fig:6dadvantage}
\end{wrapfigure}{}

\subsection{Simulation Experiments}
\begin{table}[b]
\begin{footnotesize}
\setlength{\belowcaptionskip}{-0.5cm}
\vspace{-0.4cm}
\renewcommand\arraystretch{1.2}
    \centering
    \begin{tabular}{r|cc|cc}
        \toprule
        &\multicolumn{2}{c|}{\textbf{w/o Noise}} &\multicolumn{2}{c}{\textbf{ w/ Noise}} \\
        \hline
        & Antipodal Score    & Collision-free &   Antipodal Score    & Collision-free \\
        \hline
        GPD (3 channels)   &  0.5947 &  \textbf{47.07\%} &  0.5802  & 40.00\%    \\
        GPD (12 channels)   &  0.5883  &  45.27\%  &  0.5946  & 40.44\%    \\
        PointNetGPD    &  0.5718   &  42.41\%  & 0.6376   &  41.17\%   \\
        \hline
        Ours & \textbf{0.7364}    & 47.02\%  &\textbf{0.7354}  & \textbf{53.32\%} \\
        \bottomrule   
    \end{tabular}
    \caption{Comparison of grasp quality on simulation data.}
    \label{tab:simul}
\end{footnotesize}
\end{table}

GPD~\citep{ten2017grasp} and PointNetGPD~\citep{liang2019pointnetgpd} adopt Darboux frame analysis to sample grasp poses and train a classifier to evaluate their quality, which achieved state-of-the-art performance in 6D grasp detection. We choose GPD(3 channels), GPD(12 channels), and PointGPD as our baseline methods.
% \begin{wrapfigure}{R}{0.45\textwidth}
% \begin{subfigure}[t]{0.22\textwidth}
% % \label{fig:failure_cases1}
%     \centering
%     \includegraphics[width=\textwidth]{imgs/low_score.eps}
%     \caption{}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.22\textwidth}
% % \label{fig:failure_cases2}
%     \centering
%     \includegraphics[width=\textwidth]{imgs/collision.eps}
%     \caption{}
% \end{subfigure}
% \caption{Illustration of different failure cases, (a) low antipodal score, (b) collision with objects invisible to the depth sensor.}
% \label{fig:failure_cases}
% \end{wrapfigure}
For training baseline methods, we adopt their grasp sampling strategy to generate grasp candidates for each scene until we get 300 collision-free grasps. We generate grasps over 6.5k scenes and get more than 2M grasps, which is larger than the 300K grasps in the original paper. Note that the scene used to generate training data for baseline method is exactly the same as our method.

For evaluation of baseline methods, we first sample 1000 points at random from the point cloud and calculate the Darboux frame for grasp candidates, which are then classified and ranked. The top 10 grasps are evaluated for both baseline methods and our methods.

To evaluate our method in finding collision-free grasps, we compare two metrics that affect the final grasping success rate: \textbf{(1)} antipodal score, which describes the force closure property of grasps, \textbf{(2)} probability of collision with other objects not observable to the depth sensor. The evaluation is performed in simulator with 2 settings: \textbf{(1)} No noise, where the point cloud from the depth sensor simulator aligns with the complete point cloud perfectly; \textbf{(2)} With noise, where the noise of the depth simulator is proportional to the depth. Please note that for noise setting and real-world experiment, both baselines and our method is trained on noisy data. Table.~\ref{tab:simul} shows the comparison results. Since the 6-DoF grasp pose is regressed by our \net~instead of being computed from local normals and curvatures, it is less sensitive to partial and noisy depth observations; also, our \net~is able to generate more collision-free grasps by inferring from local and global geometry information jointly.




% \begin{wrapfigure}{R}{0.45\textwidth}
% \begin{subfigure}[t]{0.22\textwidth}

%     \centering
%     \includegraphics[width=\textwidth]{imgs/robot_exp.pdf}
%     \caption{Grasping experiment setting with a Kinova Jaco2 arm}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{imgs/objects.eps}
%     \caption{Objects used in our experiments}
% \end{subfigure}
% \caption{Robotic Grasp Experiments}
% \label{fig:robotic_exp}
% \end{wrapfigure}

% \begin{table}[!t]
%     \centering
%     \setlength{\tabcolsep}{3mm}
%     \begin{tabular}{c|cccccc}
%     \toprule
%          \textbf{Direction}& $(0^{\circ} , 15^{\circ})$&$(0^{\circ} , 30^{\circ})$&$(0^{\circ} , 45^{\circ})$&$(0^{\circ} , 60^{\circ})$&$(0^{\circ} , 75^{\circ})$&$(0^{\circ} , 90^{\circ})$ \\
%          \hline
%          Simple Scene & $66.55$ & $79.93$&  $87.64$&  $93.91$&  $97.55$&  $99.98$ \\
%          Semi-Dense Scene & $61.81$ & $76.72$&  $85.97$&  $93.14$&  $96.95$& $99.98$ \\
%          Dense Scene & $57.21$ & $73.27$&  $84.17$&  $90.33$&  $95.16$&  $99.97$ \\
%          \hline
%          \textbf{Over All} & $63.38$ & $77.74$&  $86.51$&  $93.43$&  $97.22$&  $99.98$ \\
%          \bottomrule
%     \end{tabular}
%     \caption{Results of simulated experiment on the recall rate of different grasp. The direction is the angle between the approach vector and vertical direction. The angle of absolute 3/4 DoF grasp is $0^{\circ}$}
%     \label{tab:se3}
% \end{table}{}


\subsection{Robotic Experiments}

We validate the effectiveness and reliability of our methods in real robotic experiments. We carried out all the experiments on Kinova MOVO, a mobile manipulator with a Jaco2 arm attached with a 2-finger gripper (Fig.~\ref{fig:pipeline} (a)). In order to be close to real domestic robot application scenarios, we use one KinectV2 depth sensor that is mounted on the head of the manipulator, which makes the observation heavily occluded and raises the difficulty of experiments. 30 objects of various shapes and weight (see Supplymentary Materials) are used, which are absent in the training dataset. 

The experiment procedure is as follows: \textbf{(1)} Choose 10 out of the 30 objects at random and put them on the table to form a cluttered scene; \textbf{(2)} The robot attempts multiple grasps, until all objects are grasped or 15 grasps have been attempted; \textbf{(3)} Step (1) and (2) are repeated for 4 times for each method. More details are presented in the supplementary material. Note that all the objects selected in real robot experiments are out of the training data.

As illustrated in Table~\ref{tab:robot}, our method outperforms baseline methods in terms of \textit{success rate}, \textit{completion rate}, and time efficiency, which suggests that the single-shot regressed 6-DoF grasps have better force closure quality than sampled grasps from baselines, as demonstrated in Fig.~\ref{fig:sample_grasp}. Not needed by us, the baseline methods also need to detect collision and extract local geometry for every sampled grasp, which takes around 20 seconds, so they are much more time-consuming than our method. 

Our experiment setting is much more challenging than the baseline papers. In the original paper, GPD uses two depth sensors at both sides of the arena to capture the nearly complete point cloud in the original paper, but in our experiments, only one depth sensor is used. In both baselines, grasps are sampled in the neighbourhood of Darboux frame. It performs well on convex objects (box and ball) but poorly on non-convex or thin-structure objects, such as mug and bowl as in our experiments, because their heuristic sampling method requires accurate normals and curvatures but estimating those surface normals from noisy point cloud is challenging. On the contrary, Point-Net++ has been demonstrated to be robust against adversarial changes to the input data \cite{liu2019extending}, which can better capture the geometric structure under noise.


\begin{table}[]
\setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \setlength{\belowcaptionskip}{-0.5cm}
    \setlength{\tabcolsep}{2.5mm}{
    \begin{tabular}{r|cc|ccc}
        \toprule
         &\multicolumn{2}{c|}{\textbf{Grasp quality}} &\multicolumn{3}{c}{\textbf{Time-efficiency}} \\
        \hline
            & Success rate  & Completion rate & Processing & Inference &\textbf{ Total}  \\
        \hline
        GPD (3 channels)   &  40.0\%  &  60.0\%  &  24106 ms   &  \textbf{1.50 ms}   & 24108 ms    \\
        GPD (12 channels)   &  33.3\%  & 50.0\%  & 27195ms  & 1.70ms &  27197ms \\
        PointNetGPD  &  40.0\%  &  60.0\%  &  17694ms  &  2.86ms    & 17697ms  \\
        \hline
        Ours& \textbf{77.1\%} & \textbf{92.5\%} & \textbf{5804ms} & 12.60 ms & \textbf{5817 ms}\\
        \bottomrule   
    \end{tabular}}
    \caption{Results of robotic experiments on dense clutters. \textit{Success rate} and \textit{completion rate} are used as the evaluation metrics, which represent the accuracy and completeness respectively. }
    \label{tab:robot}
\end{table}

\begin{figure}[b]
\setlength{\belowcaptionskip}{-0.5cm}
\vspace{-0.4cm}
\centering
    \includegraphics[width=1\linewidth]{imgs/sample_grasp.pdf}
    \caption{Comparison between sampled grasps chosen by baseline methods with high-score and regressed grasps by our method. }
    \label{fig:sample_grasp}
\end{figure}


==> [Arxiv]Grasp Proposal/relate.tex <==
\section{Related work}
% \hao{ddl: 9pm, Meng}
% \paragraph{Classical 6-DoF Grasping Methods}
%\paragraph{Deep Learning based Grasping Methods}
%\paragraph{Training Data Synthesis for Grasping}
%\paragraph{Deep Learning on 3D Data}

\paragraph{Deep Learning based Grasping Methods}
\citet{caldera2018review} gave a thorough survey of deep learning methods for robotic grasping, which demonstrates the effectiveness of deep learning on this task. In our paper, we focus on the problem of 6-DoF grasp proposal. \citet{collet2011moped, zeng2017multi, mousavian20196} tackled this problem by fitting the object model to the scan point cloud to retrieve the 6-DoF pose. Although it has shown promising results in industrial applications, the feasibility is limited in generic robotic application scenarios, e.g. house-holding robots, where the exact 3D models of numerous objects are not accessible. \citet{ten2017grasp} proposed to generate grasp hypotheses only based on local geometry prior and attained better generalizability on novel objects, which was further extended by~\citet{liang2019pointnetgpd} by replacing multi-view projection features with direct point cloud representation. Because potential viable 6-DoF grasp poses are infinite, these methods guide the sampling process by constructing a Darboux frame aligned with the estimated surface normal and principal curvature and searching in its 6D neighbourhood. However, they may fail finding feasible grasps for thin structures, such as plates or bowls, where computing normals analytically from partial and noisy observation is challenging. In contrast to these sampling approaches, our framework is a single-shot grasp proposal framework~\citep{chu2018real, caldera2018review}--a direct regression approach for predicting viable grasp frames--which could handle flawed input well due to the network's knowledge. Moreover, by jointly analyzing local and global geometry information, our method not only considers the object of interest, but also its surroundings, which allows the generation of collision-free grasps in dense clutters. 

\paragraph{Training Data Synthesis for Grasping}
Deep learning methods require an enormous volume of labelled data for the training process~\citep{kumra2017robotic}, however manually annotating 6-DoF grasp poses is not practical. Therefore, analytic grasp synthesis~\citep{bicchi2000robotic} is indispensable for ground truth data generation. These advanced models have provided guaranteed measurements of grasp properties with the availability of complete and precise geometric models of objects. In practice, the observation from sensors are partial and noisy, which undermines the metric accuracy. In the service of our single-shot grasp detection framework, we first use analytic methods to generate viable grasps for each single object, and reject unfeasible grasps in densely clutter scenes. To the best of our knowledge, the dataset we generated is the first large-scale synthetic 6-DoF grasp dataset for dense clutters.

\paragraph{Deep Learning on 3D Data}

\citet{qi2016pointnet, qi2017pointnet++} proposed PointNet and PointNet++, a novel 3D deep learning network architecture capable of extracting useful representations from 3D point clouds. Compared with other architectures~\citep{maturana2015voxnet, qi2016volumetric}, PointNets are robust to varying sampling densities, which is important to real robotic applications. In this paper, we utilize PointNet++ as the backbone of our single-shot grasp detection and demonstrate its effectiveness.
